Sim-to-Real Strategy for Spatially Aware Robot Navigation in Uneven Outdoor Environments

Deep Reinforcement Learning (DRL) is hugely successful due to the availability of realistic simulated environments. However, performance degradation during simulation to real-world transfer still remains a challenging problem for the policies trained in simulated environments. To close this sim-to-real gap, we present a novel hybrid architecture that utilizes an intermediate output from a fully trained attention DRL policy as a navigation cost map for outdoor navigation. Our attention DRL network incorporates a robot-centric elevation map, IMU data, the robot's pose, previous actions, and goal information as inputs to compute a navigation cost-map that highlights non-traversable regions. We compute least-cost waypoints on the cost map and utilize the Dynamic Window Approach (DWA) with velocity constraints on high cost regions to follow the waypoints in highly uneven outdoor environments. Our formulation generates dynamically feasible velocities along stable, traversable regions to reach the robot's goals. We observe an increase of 5% in terms of success rate, 13.09% of the decrease in average robot vibration, and a 19.33% reduction in average velocity compared to end-to-end DRL method and state-of-the-art methods in complex outdoor environments. We evaluate the benefits of our method using a Clearpath Husky robot in both simulated and real-world uneven environments.

==> 2_Related_Work.tex <==
\section{Related Work}
\subsection{Sim-to-Real Solutions for Navigation}
\subsection{Robot Navigation in Unstructured Environments }

==> 3_Background.tex <==
\section{Background}

